The AdobeIndoorNav Dataset: Towards Deep Reinforcement Learning based Real-world Indoor Robot Visual Navigation

Deep reinforcement learning (DRL) demonstrates its potential in learning a model-free navigation policy for robot visual navigation. However, the data-demanding algorithm relies on a large number of navigation trajectories in training. Existing datasets supporting training such robot navigation algorithms consist of either 3D synthetic scenes or reconstructed scenes. Synthetic data suffers from domain gap to the real-world scenes while visual inputs rendered from 3D reconstructed scenes have undesired holes and artifacts. In this paper, we present a new dataset collected in real-world to facilitate the research in DRL based visual navigation. Our dataset includes 3D reconstruction for real-world scenes as well as densely captured real 2D images from the scenes. It provides high-quality visual inputs with real-world scene complexity to the robot at dense grid locations. We further study and benchmark one recent DRL based navigation algorithm and present our attempts and thoughts on improving its generalizability to unseen test targets in the scenes.

==> tex/method.tex <==
In the pioneering work \cite{zhu2017target}, they formulate the robot indoor navigation problem as a target-driven deep reinforcement learning task. Conditioned on a given target objective, the robot directly predicts an action at every location from the visual observation. The success of training such DRL based models opens up a promising direction for the research in map-less robot visual navigation.

To review the DRL based method proposed in \cite{zhu2017target}, they train a siamese Asynchronous Advantange Actor-Critic (A3C) models \cite{mnih2016asynchronous} that takes both the current observation and the target view as inputs and predicts an action among the four actions to take (i.e. go forward, go backward, turn left and turn right). Both observation images are represented by a 2,048-dim image feature extracted from an ImageNet-pretrained ResNet \cite{he2016deep}. The networks are trained on millions of episodes simulated on the AI2-THOR synthetic scenes \cite{kolve2017ai2}. Instead of explicitly maintaining a belief for the scene map, the A3C networks learn latent spatial layouts for navigation. Scene-specific layers are introduced to better encode the room layouts for different scenes.

It is interesting to observe that the proposed target-driven DRL model demonstrates its ability to navigate solely based on the current visual input and a target image. Unfortunately, a thorough study reveals that the method suffers from target generalization problem. The learned A3C models are able to navigate to the targets that have been seen during training or are close to one of the train targets in near shortest paths. However, when navigating to test targets that are far from the train targets, the models fail quickly and even cannot reach the final targets. The target generalization issue limits the method to be applied to the real-world scenarios. In this section, we propose to use dense target training and spatial-aware feature to address the target generalization problem.

\subsection{Dense-target Training}
Despite of its strong capability to navigate to the train targets, the A3C models proposed in \cite{zhu2017target} fails to generalize to the unseen test targets. In their experiments, they train the model on 8 landmark targets and test its performance on navigating to test targets that are few steps away from the train targets. They set the maximum number of steps to be 500 for each episode. Experiments show that the success rate quickly drops from near 100\% on the train targets to around 70\%, 40\%, 34\%, below 29\% on the test targets that are 1, 2, 4 and 8 steps away.

This fact reveals that the proposed A3C method \cite{zhu2017target} suffers from the target generalization issue. Their method learns the  observation feature embedding that overfits to the train targets and fails to generalize to the other targets that are unseen during training. To address the issue, we propose to sample dense training targets from all targets that have distinctive image features and train A3C models on all the selected targets. For each scene, instead of just training the agent to navigate to only $5\sim10$ selected landmark target views, we train a model on densely sampled target locations across the entire scenes. By using dense-target training, the models are expected to learn better holistic room layout embedding and avoid the overfitting to the landmark targets. Experiments show that we learn a model that generalizes to unseen targets much better.

\subsection{Spatial-aware Feature}
Experiments show that dense-target training significantly improves the target generalization of the A3C models. However, it slows down the training procedure because the A3C models are trained for substantially more targets than the selected landmarks, which makes the training harder to converge. In this section, we study the common navigation failure cases and propose to use spatial-aware feature to speed up the training procedure.

Fig. \ref{fig:method_spatial_aware_fail} shows the common failure case that we obtains from training an A3C model on the \textit{et12-kitchen} and testing it on the unseen targets. We train the model on sparsely sampled landmark targets only and evaluate on the other locations with distinctive image features. For all of the four examples, the agent finally fails to reach the targets but it indeed reaches the nearby locations with similar views. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/method_spatial_aware_fail.pdf}
    \caption{Navigation Failure Examples. For each pair of images, the left one shows the current observation and the right image is the target view. In these examples, the agent finally does not reach the target even the current view is very similar to the target view.}
    \label{fig:method_spatial_aware_fail}
\end{figure}

We observe that the learned model behaves clearly in two stages. Starting from a random location, the agent quickly navigates to the area around the test target in a few steps. This behavior shows that the model successfully learns a rough room layout and uses it for navigation. However, after reaching the nearby area, the agent begins to vacillate around the target location and finally fails to locate the exact target view. The potential reason for this behavior is that the room layout embedding is trained on the sparse train targets only and it is not accurate for the unseen targets. Also, the network lacks the ability to do image feature matching and discriminate local spatial relationship between similar views.

To address this issue, we propose to use spatial-aware feature for image representation. Spatial-aware features encode more spatial information that is crucial for image matching between two similar views and local spatial reasoning in the underlying 3D scene. In \cite{zhu2017target}, they use an Imagenet-pretrained ResNet network \cite{he2016deep} to extract features for the observations. Each image is represented by a 2,048-dim feature extracted from the second to the last layer right before the final classification layer. 

The 2,048-dim feature lacks the spatial information on the image space because the prior pooling layers remove such knowledge. In our method, we propose to use the $7\times7\times2,048$ spatial-aware feature right before the last pooling layer to represent the image features. Experiments show that the proposed spatial-aware features encode more spatial information which is crucial for image matching. Also, using better image features as inputs, the A3C models converge significantly faster than the models trained with 2,048-dim image features.
